Finding Nontrivial Minimum Fixed Points in Discrete Dynamical Systems

Networked discrete dynamical systems are often used to model the spread of contagions and decision-making by agents in coordination games. Fixed points of such dynamical systems represent configurations to which the system converges. In the dissemination of undesirable contagions (such as rumors and misinformation), convergence to fixed points with a small number of affected nodes is a desirable goal. Motivated by such considerations, we formulate a novel optimization problem of finding a nontrivial fixed point of the system with the minimum number of affected nodes. We establish that, unless P = NP, there is no polynomial time algorithm for approximating a solution to this problem to within the factor n^1-\epsilon for any constant epsilon > 0. To cope with this computational intractability, we identify several special cases for which the problem can be solved efficiently. Further, we introduce an integer linear program to address the problem for networks of reasonable sizes. For solving the problem on larger networks, we propose a general heuristic framework along with greedy selection methods. Extensive experimental results on real-world networks demonstrate the effectiveness of the proposed heuristics.

==> tex/titlepage.tex <==
% !TEX root = ./main.tex

\begin{titlepage}

{

%\center{\textcolor{red}{For Evaluation By PKDD Only --- Not for Public Use/Consumption\\
%To be Released at a Later Date}}

\normalsize
\rightline{\bf NDSSL Technical Report 2017-1035}
%\medskip
\vspace{0.2in}
\normalsize{\hfill{Sept. 17, 2017}}

\vspace{0.05in}
\noindent\begin{tabular}{r|p{0.75\textwidth}}
\rule[0.25in]{0pt}{0pt} & \\
Title:&\normalsize{Learning and Inference in Networked Social Systems -- Part 2:} \\
      &\normalsize{Deterministic Query Generation Methods} \\
\rule[0.5in]{0pt}{0pt} & \\
Authors: &
\small{
Abhijin Adiga\newline
Christopher J. Kuhlman\newline
Madhav V. Marathe\newline
S. S. Ravi\newline
Daniel J. Rosenkrantz\newline
Richard E. Stearns}\\

%\institute{
%Virginia Bioinformatics Institute, Virginia Tech, Blacksburg, 
%VA 24061, USA.
%Email:~ \texttt{\{ckuhlman,akumar,mmarathe\}@vbi.vt.edu} \\ \and
%Computer Science Department, University at Albany -- SUNY, 
%Albany, NY 12222, USA.
%Email:~ \texttt{\{ravi,djr\}@cs.albany.edu}
%}

\rule[0.25in]{0pt}{0pt} & \\
Contact: &
\small{Madhav V. Marathe\newline
 Email: {\tt mmarathe@bi.vt.edu} \newline
 Tel.: +1 540 231 8832\newline
 Fax: +1 540 231 2891} \\
\rule[0.25in]{0pt}{0pt} & \\

%To Appear In: &
%%Submitted To: &
%\small{The 10th IEEE International Conference on e-Science (eScience 2014)}\\
%%\small{}\\


\rule[0.25in]{0pt}{0pt} & \\
Acknowledgments: & \small{
We convey our special thanks to 
Noshir Contractor (Northwestern University),
Joshua Epstein (New York University),
Brian Goode (Virginia Tech),
Michael Macy (Cornell University), 
Naren Ramakrishnan (Virginia Tech) and
Nathan Self (Virginia Tech)
for discussions on topics related to the paper.
This work has been partially supported by
DARPA Cooperative Agreement D17AC00003 (NGS2),
DTRA CNIMS (Contract HDTRA1-11-D-0016-0001),
NSF DIBBS Grant ACI-1443054 and
NSF BIG DATA Grant IIS-1633028.
The U.S. Government is authorized to reproduce and
distribute reprints for Governmental purposes notwithstanding
any copyright annotation thereon.

\bigskip

\noindent
\textbf{Disclaimer:}~ The views and conclusions contained herein are those 
of the authors and should
not be interpreted as necessarily representing the 
official policies or endorsements, either expressed
or implied, of DARPA or the U.S. Government.
} \\
\rule[0.25in]{0pt}{0pt} & \\
\end{tabular}

\vfill

\rightline{\makebox[3.5in][l]{\vbox{\small
\noindent Network Dynamics and Simulation Science Laboratory\\
Biocomplexity Institute of Virginia Tech\\
Virginia Polytechnic Institute and State University\\
%%and\\
%%Computer Science Department, University at Albany -- SUNY
}}}

%\noindent\includegraphics[width=\textwidth]{VBI_VT_Logo.eps}
\title{}
\author{}
\date{}

%\textcolor{red}{For Evaluation By PKDD Only --- Not for Public Use/Consumption}

}

\bigskip\bigskip

\begin{center}
\fbox{\fbox{\Large{\textbf{Preliminary Version:~ Please Do Not Distribute}}}}
\end{center}

\thispagestyle{empty}

\end{titlepage}

